Community Recovery in the Geometric Block Model

To capture the inherent geometric features of many community detection problems, we propose to use a new random graph model of communities that we call a Geometric Block Model. The geometric block model builds on the random geometric graphs (Gilbert, 1961), one of the basic models of random graphs for spatial networks, in the same way that the well-studied stochastic block model builds on the Erd\H{o}s-R\'{en}yi random graphs. It is also a natural extension of random community models inspired by the recent theoretical and practical advancements in community detection. To analyze the geometric block model, we first provide new connectivity results for random annulus graphs which are generalizations of random geometric graphs. The connectivity properties of geometric graphs have been studied since their introduction, and analyzing them has been more difficult than their Erd\H{o}s-R\'{en}yi counterparts due to correlated edge formation. We then use the connectivity results of random annulus graphs to provide necessary and sufficient conditions for efficient recovery of communities for the geometric block model. We show that a simple triangle-counting algorithm to detect communities in the geometric block model is near-optimal. For this we consider the following two regimes of graph density. In the regime where the average degree of the graph grows logarithmically with the number of vertices, we show that our algorithm performs extremely well, both theoretically and practically. In contrast, the triangle-counting algorithm is far from being optimum for the stochastic block model in the logarithmic degree regime. We simulate our results on both real and synthetic datasets to show superior performance of both the new model as well as our algorithm.

==> gbm-dense.tex <==

\section{ High dimensional GBM in dense graphs}
\label{appen:dense}
In Section~\ref{sec:sparse-high} and Section~\ref{sec:rag} we  analyzed the algorithm and connectivity conditions for logarithmic regime. In this section, we explore the dense regime for $r_s$ and $r_d$. In that case, the number of edges in the graph can be of the order of $O(n^2)$\footnote{When $r_s$ and $r_d$ are constant values}. For processing and computing efficiency, it is much desirable if we can just use a subset of $O(n\log{n})$ edges and determine the communities. In this section, we give such an algorithm which does not even look at the entire graph and returns the communities.

The algorithm runs in two phases. In the first phase we sample $h(n)$ nodes randomly from the entire set of vertices $V$. We denote this set of sampled vertices as $C$ and subsequently we run the algorithm \texttt{process} described before on $C$ with suitable thresholds  for $E_S$ and $E_D$ to cluster these $h(n)$ nodes. In the second phase we sample $g(n)$ nodes from each cluster of $C$. Now, for each of the remaining unresolved $n-h(n)$ nodes, we calculate its neighbors in the sampled $g(n)$ nodes from each cluster in $C$. We include the node to the cluster for which it has more neighbors (in the sampled $g(n)$ nodes).  Thus the number ofclose). Table I describes the number of edges across the communities. It is evident that the authors from same community are edges we need to see to classify the entire set of vertices is $O(ng(n)+h(n)^{2})$.  $h(n)$ and $g(n)$ is naturally a function of $r_s$, $r_d$ and dimension $t$. The goal is to select $h(n)$ and $g(n)$ as small as possible. We set  $g(n) =\min\{\frac{n}{2},\log n \Big(\frac{\sqrt{12B_t(r_d)}+\sqrt{12B_t(r_s)}}{B_t(r_s)-B_t(r_d)}\Big)^{2}\}$and 
$h(n)=\min\{n,O(\sqrt{ng(n)})\}$. We set $E_S = \theta^t_S(B_t(r_d)h(n)+\sqrt{6B_t(r_d) h(n)\log n})$ and $E_D = \theta^t_D( h(n)\mathcal{V}_t(r_s,r_d,r_d)-\sqrt{6h(n)B_t(r_d)\log n })$ where $\theta^t_S > 1$ and $\theta^t_D < 1$ are constants chosen suitably.
%The pseudocode for {\em Cluster recovery in Dense GBM} is given below.



%\captionof{algorithm}{Cluster recovery in Dense GBM}
%\begin{algorithmic}[1]\label{alg:alg1d}
%{
%\REQUIRE GBM $V$, $r_s, r_d$
%\STATE $g(n) \leftarrow (\sqrt{12r_d/r_s} + 2\sqrt{2}) \frac{r_s \log n}{ (r_s-r_d)^2}$  \hfill $\blacktriangleright$ {Setting sampling  parameters}
%\STATE $h(n) \leftarrow \sqrt{ng(n)}$
%\STATE $C\leftarrow \texttt{sample}(V,h(n)) $
%\STATE $E' \leftarrow \{(u,v) \mid u, \in C, (u,v)\in E \}$ \hfill  $\blacktriangleright$ {Identify the edges within $C$}
%%\FOR {$u\in C$}
%%\FOR {$v\in C\setminus \{u\}$}
%%\IF {$\texttt{query}(u,v)$}
%%\STATE $E' \leftarrow E'\cup \{(u,v)\}$ 
%%\ENDIF
%%\ENDFOR
%%\ENDFOR
%\STATE $C_1,C_2\leftarrow \texttt{RunMotifCount}(C,E', r_s, r_d)$ \hfill  $\blacktriangleright$ {Cluster $C$ using triangle count algorithm}
%\STATE$ S\leftarrow \texttt{sample}(C_1,g(n))$ \hfill $\blacktriangleright$ {Second Phase starts here}
%\FOR {$ u \in V\setminus C$}
%\STATE $deg_u^S \leftarrow | \{(u,v)\mid v\in S, (u,v)\in E\}| $ \hfill  $\blacktriangleright$ {Degree calculation with $S$}
%%\FOR {$ v \in S$}
%%\STATE $deg_u^S\leftarrow 0$
%%\IF{\texttt{query}(u,v)}
%%\STATE $deg_u^S\leftarrow deg_u^S + 1$
%%\ENDIF
%%\ENDFOR
%\IF { $|deg_u^S - \Delta_S | \leq | deg_u^S - \Delta_D |  $} 
%\STATE \hfill $\blacktriangleright$ {Threshold degree of $u$ with the nodes of $S$ to identify the cluster}
%\STATE $C_1 \leftarrow C_1 \cup \{u\}$
%\ELSE
%\STATE $C_2 \leftarrow C_2 \cup \{u\}$
%\ENDIF
%\ENDFOR
%\RETURN $C_1,C_2$\\
%}
%\end{algorithmic}
%\end{algorithm}
%\end{minipage}


%
%\begin{lemma}[Chernoff Bound]
%Let $X_1, \ldots, X_n$ be iid random variables in $\{0,1\}$. Let $X$ denote the sum of these $n$ random variables. Then for any $\delta>0$,
%\[
% \begin{cases}
%\Pr(X > (1+\delta) \avg(X)) \le e^{-\delta^2\avg(X)/3}  = \frac{1}{n\log^2 n}, \text{ when } \delta = \sqrt{\frac{3(\log{n}+2\log\log n)}{\avg(X)}}.\\
%\Pr(X < (1-\delta)\avg(X)) \leq e^{-\delta^2\avg(X)/2} = \frac{1}{n\log^2 n},\text{ when } \delta = \sqrt{\frac{2(\log{n}+2\log\log n)}{\avg(X)}}
%\end{cases}
%\]
%\end{lemma}
%

\subsection{Analysis.}
Recall that in the first phase of the algorithm, we sample $h(n)=\Omega(\log n)$ nodes at random. Assume that $c_1$ nodes out of those $h(n)$ nodes belong to cluster $C_1$ and $c_2$ nodes  belong to cluster $C_2$. Of course, we must have that $c_1+c_2=h(n)$.
\begin{lemma}\label{lem:sample}
In the first phase of the algorithm on sampling $C, |C| = h(n)$ nodes, the number of nodes belonging to each cluster satisfies

$$ h(n)/2 - \sqrt{6h(n)\log n}  \leq c_1 \leq  h(n)/2   + \sqrt{6h(n)\log n} \text{ and }$$ 
$$ h(n)/2 - \sqrt{6h(n)\log n}  \leq c_2 \leq  h(n)/2   + \sqrt{6h(n)\log n}$$ 
with probability of at least $1-\frac{2}{n^2\log^2n}$.
\end{lemma}
\begin{proof}
The statement follows simply by applying the Chernoff bound and then a union bound over the two clusters. 
%Specifically, 
%define for each $u \in C$, $X_u$ to be an indicator random variable which is $1$ when $u \in C_1$ and $0$ otherwise (similarly for $C_2$).
%Using the Chernoff bound, with probability of at lease $1-\frac{1}{n^2\log^2n}$
%\begin{align*}
%\Pr(\sum_{u\in C} X_u ) \leq  h(n)/2+ \sqrt{6h(n)\log n} 
%\end{align*}
%Similarly, with a probability of at least $1-\frac{1}{n^2\log^2n}$
%\begin{align*}
%\Pr(\sum_{u\in C} X_u ) \geq  h(n)/2- \sqrt{6h(n)\log n} 
%\end{align*}
%Hence, $$ h(n)/2 - \sqrt{3h(n)\log n}  \leq |C_1| \leq  h(n)/2   + \sqrt{3h(n)\log n}$$ with a  probability of at least $1-\frac{2}{n^2\log^2n}$.
\end{proof}




The proof of correctness of the first phase of the algorithm is similar to the proof of sparse regime as discussed in Section \ref{sec:sparse-high}. Let us set $E_S = \theta_S(B_t(r_d)h(n)+\sqrt{6B_t(r_d) h(n)\log n})$ and $E_D = \theta_D( h(n)\mathcal{V}_t(r_s,r_d,r_d)-\sqrt{6h(n)B_t(r_d)\log n })$ where $\theta_S > 1$ and $\theta_D < 1$ are suitable constants to be chosen later.


\begin{lemma}
\label{lem:diff}
For any pair of nodes $u,v \in C, (u,v)=e\in E,\  u \nsim v$, the \texttt{process} algorithm removes the edge $e$ with a probability of $1-O\left(\frac{1}{n^2\log^2 n}\right)$. 
\end{lemma}



\begin{proof}
Let $Z$ denote the random variable corresponding to the number of common neighbors of $u,v \in V: (u,v) \in E$. Let $d(u,v) = \ell$. From Lemma \ref{lem:sep2d}, $E[Z]\leq(h(n) -2)B_t(r_d)$. Using the Chernoff bound, with probability at least $1-O\Big(\frac{1}{n^2\log^2 n}\Big)$
\begin{align*}
Z\le &\  (h(n) -2)B_t(r_d) + \sqrt{3(2\log n+ \log \log n)(h(n)-2)B_t(r_d) }\\
=& \  B_t(r_d)h(n)+(\sqrt{6B_t(r_d)} +o(1))\sqrt{h(n)\log n}\\
\geq & \  E_S
\end{align*}
Moreover again from Lemma~\ref{lem:sep2d}, $E[Z]=(h(n)-2)\min(\mathcal{V}_t(r_s,r_d,\ell),B_t(r_d))$. Hence, with probability of at least $1-O\Big(\frac{1}{n^2\log^2 n}\Big)$
\begin{align*}
Z\ge &\ \min_{\ell: \ell \le r_d,r_s \le 2r_d} ( ( h(n) -2)\min(\mathcal{V}_t(r_s,r_d,\ell),B_t(r_d)) - \\
  & \sqrt{3(2\log n+ \log \log n)(h(n)-2)\min(\mathcal{V}_t(r_s,r_d,\ell),B_t(r_d)) }) \\
%=& \  \min_{r_s-r_d \leq x \leq r_d}(r_s+r_d-x)h(n)- (\sqrt{4(r_s+r_d-x)} +o(1))\sqrt{h(n) \log n}\\
%&\text{SINCE WE DONT CARE OF CONSTANTS }\\
\geq & h(n)\mathcal{V}_t(r_s,r_d,r_d)-\sqrt{6h(n)B_t(r_d)\log n } \\
\geq & \  E_D
\end{align*}

Here the second inequality followed from the fact that $\mathcal{V}_t(r_s,r_d,\ell) \leq B_t(r_d)$ and $\mathcal{V}_t(r_s,r_d,\ell)$ is a decreasing function of $\ell$.
\end{proof}

Hence, on taking a union bound over all intercluster edges  $ u,v \in h(n),(u,v) \in E$ (at most ${n \choose 2}$), the triangle count must be within $E_S$ and $E_D$ for all such edges with a probability of at least $1-O\Big(\frac{1}{\log n}\Big)$. Thus all the intercluster edges will be removed with probability $1-o(1)$. 


\begin{lemma}
\label{lem:essame-2}
Given a pair of nodes $u,v$ belonging to the same cluster such that $(u,v) \in E$, the \texttt{process} algorithm does not remove the edge $e$ with probability of $1-O\left( \frac{1}{n\log^2 n}\right)$ when $d(u,v)=\ell$ (say) satisfies the following:
\begin{align*}
\frac{h(n)}{2}\Big(\mathcal{V}_t(r_s,r_s,\ell)+\mathcal{V}_t(r_d,r_d,\ell)\Big)- \sqrt{25h(n)\log{n}}\Big(\sqrt{B_t(r_s)} + \sqrt{B_t(r_d)} \Big) > E_S \tag{D1}
\end{align*}  
\end{lemma}
\begin{proof}
Let $Z$ denote the random variable corresponding to the number of common neighbors of $u,v$. Let $\mu_s(\ell)= \avg(Z|u \sim v, d(u,v)=\ell)$. From Lemma~\ref{lem:sepd}, $\mu_s(\ell)=(c_1-2)\cV(r_s,r_s,l)+c_2\cV(r_d,r_d,l)$.

Using the Chernoff bound, with a probability of $1-O\Big(\frac{1}{n^2\log^2 n}\Big)$

\begin{align*}
Z \geq &
 c_1\mathcal{V}_t(r_s,r_s,\ell)+c_2\mathcal{V}_t(r_d,r_d,\ell)  - \sqrt{3(2\log n+\log\log n)\mathcal{V}_t(r_s,r_s,\ell)c_1}    \\&- \sqrt{3(2\log n+\log\log n)\mathcal{V}_t(r_d,r_d,\ell)c_2}\\
 & \geq c_1\mathcal{V}_t(r_s,r_s,\ell)+c_2\mathcal{V}_t(r_d,r_d,\ell)  - \sqrt{3(2\log n+\log\log n)\mathcal{V}_t(r_s,r_s,\ell)h(n)}    \\&- \sqrt{3(2\log n+\log\log n)\mathcal{V}_t(r_d,r_d,\ell)h(n)}\\
&=\frac{h(n)}{2}\Big(\mathcal{V}_t(r_s,r_s,\ell)+\mathcal{V}_t(r_d,r_d,\ell)\Big)-\sqrt{6h(n)\log{n}}\Big(\mathcal{V}_t(r_s,r_s,\ell)+\mathcal{V}_t(r_d,r_d,\ell)\Big) \\
& -(\sqrt{\mathcal{V}_t(r_s,r_s,\ell)} + \sqrt{\mathcal{V}_t(r_d,r_d,\ell)} )\sqrt{12h(n)\log n}\\
& \geq \frac{h(n)}{2}\Big(\mathcal{V}_t(r_s,r_s,\ell)+\mathcal{V}_t(r_d,r_d,\ell)\Big)-\sqrt{25h(n)\log{n}}\Big(\sqrt{\mathcal{V}_t(r_s,r_s,\ell)}+\sqrt{\mathcal{V}_t(r_d,r_d,\ell)}\Big)\\
& \geq \frac{h(n)}{2}\Big(\mathcal{V}_t(r_s,r_s,\ell)+\mathcal{V}_t(r_d,r_d,\ell)\Big)- \sqrt{25h(n)\log{n}}\Big(\sqrt{B_t(r_s)} + \sqrt{B_t(r_d)} \Big)
\end{align*}

Therefore,  the \texttt{process} algorithm will not delete $e$ if 
\begin{align*}
\frac{h(n)}{2}\Big(\mathcal{V}_t(r_s,r_s,\ell)+\mathcal{V}_t(r_d,r_d,\ell)\Big)- \sqrt{25h(n)\log{n}}\Big(\sqrt{B_t(r_s)} + \sqrt{B_t(r_d)} \Big) > E_S
\end{align*}
Note that there exists a maximum value of distance (referred to as $\ell_1$) such that whenever $d(u,v) \leq \ell_1$, the condition will be satisfied.

\end{proof}




%\begin{corollary}
%Let us assume  $h(n)>\Omega(\log n)$ and $r_s,r_d$ to be constants. If $\mathcal{V}_t(r_s,r_s,\ell)+\mathcal{V}_t(r_d,r_d,\ell)-2B_t(r_d)=\omega\Big(\sqrt{\frac{\log n}{h(n)}}\Big)$ then for any two nodes $u,v$ belonging to the same cluster such that $u,v \in C,(u,v) \in E$ and $d(u,v)=\ell, 0\le \ell \le \ell^{\star}$ where 
%\begin{align*}
%\ell^{\star}=\argmax_{x} \mathcal{V}_t(r_s,r_s,x)+\mathcal{V}_t(r_d,r_d,x)> 2B_t(r_d)
%\end{align*}
%the edge $(u,v)$ is not removed by \texttt{MotifCount} algorithm with probability at least $1-O\Big(\frac{1}{\log n}\Big)$. 
%\end{corollary}

%On solving these equations, we get that when $\theta \in [0,a-b)$, our algorithm can identify the intra-cluster edges correctly.

\begin{lemma}
\label{lem:edsamed-2}
Given a pair of nodes $u,v$ belonging to the same cluster such that $(u,v) \in E$, the \texttt{process} algorithm does not remove the edge $e$ with probability of $1-O\left( \frac{1}{n^2\log^2 n}\right)$ when $d(u,v)= \ell$ (say) satisfies the following:
\begin{align*}
\frac{h(n)}{2}\Big(\mathcal{V}_t(r_s,r_s,\ell+\mathcal{V}_t(r_d,r_d,\ell)\Big))+ \sqrt{36h(n)\log{n}}\sqrt{[\mathcal{V}_t(r_s,r_s,\ell)+\mathcal{V}_t(r_d,r_d,\ell)]} \leq E_D. \tag{D2}
\end{align*}\end{lemma}
\begin{proof}

Let $Z$ denote the random variable corresponding to the number of common neighbors of $u,v$. Let $\mu_s(\ell)= \avg(Z|u \sim v, d(u,v)=\ell)$. 
From Lemma~\ref{lem:sepd}, $\mu_s(\ell)=(c_1-2)\cV(r_s,r_s,l)+c_2\cV(r_d,r_d,l)$.

Using the Chernoff bound, with a probability of $1-O\Big(\frac{1}{n^2\log^2 n}\Big)$
\begin{align*}
Z &<  c_1\mathcal{V}_t(r_s,r_s,\ell)+c_2\mathcal{V}_t(r_d,r_d,\ell)  + \sqrt{3(2\log n+2\log\log n)[c_1\mathcal{V}_t(r_s,r_s,\ell)+c_2\mathcal{V}_t(r_d,r_d,\ell)]} \\
 &\le \frac{h(n)}{2}\Big(\mathcal{V}_t(r_s,r_s,\ell)+\mathcal{V}_t(r_d,r_d,\ell)\Big)+\sqrt{6h(n)\log{n}}\Big(\mathcal{V}_t(r_s,r_s,\ell)+\mathcal{V}_t(r_d,r_d,\ell)\Big)\\
 &+ \sqrt{12h(n)\log{n}}\sqrt{[\mathcal{V}_t(r_s,r_s,\ell)+\mathcal{V}_t(r_d,r_d,\ell)]}\\
&\leq \frac{h(n)}{2}\Big(\mathcal{V}_t(r_s,r_s,\ell)+\mathcal{V}_t(r_d,r_d,\ell)\Big)+ \sqrt{36h(n)\log{n}}\sqrt{[\mathcal{V}_t(r_s,r_s,\ell)+\mathcal{V}_t(r_d,r_d,\ell)]}
\end{align*}
The  \texttt{process} algorithm will not remove $e$ if 
$$ \frac{h(n)}{2}\Big(\mathcal{V}_t(r_s,r_s,\ell)+\mathcal{V}_t(r_d,r_d,\ell)\Big)+ \sqrt{36h(n)\log{n}}\sqrt{[\mathcal{V}_t(r_s,r_s,\ell)+\mathcal{V}_t(r_d,r_d,\ell)]} \leq E_D.$$ 
Note that there exists a minimum value of distance (referred to as $\ell_2$) such that whenever $d(u,v) \geq \ell_2$, the condition will be satisfied.
\end{proof}





\begin{lemma}\label{lem:main-2}
The \texttt{process} algorithm  does not remove any intra-cluster edge $(u,v)$ if it satisfies either $d(u,v) \leq \ell_1$ or $\ell_2 \leq d(u,v) \leq r_s$ with probability at least $1-O(\frac{1}{\log^2{n}})$.
\end{lemma}
\begin{proof}
The proof follows from Lemma~\ref{lem:essame-2} and Lemma~\ref{lem:edsamed-2} and applying union bound over a maximum possible of ${n}\choose{2}$ edges.
\end{proof}

Therefore, as long as $\ell_1$ and $\ell_2$ satisfies the connectivity condition of a random annulus graph (Theorem~\ref{thm:highdem1}), the clusters are correctly identified in the first phase.
%{\color{red} the RAG result needs to be changed for any value of $r_s$ and $r_d$.}

%This shows that the set of edges identified correctly by the \texttt{MotifCount} algorithm are equivalent to a random annulus graph  over the nodes of same cluster where the nodes are connected whenever the distance between the nodes follow theorem \ref{th:main1d}.


\remove{
\begin{corollary}
For given values of  $r_s$, $r_d$ with $r_s-r_d =\epsilon  $, the first phase of Algorithm \ref{alg:alg1} can successfully cluster the nodes in $C$ if $\epsilon = \Omega\left(\sqrt{\frac{r_s\log n}{n}}\right)$\end{corollary}

\begin{corollary}
When $r_s$, $r_d$ are constants with $r_s-r_d =\epsilon$, the first phase of Algorithm \ref{alg:alg1} can successfully cluster the nodes in $C$ if $\epsilon = \Omega \left(\sqrt{\frac{\log n}{n}}\right)$
\end{corollary}

\begin{corollary}
When $r_s$, $r_d$ are constants with $r_s-r_d =\epsilon  = \Omega(\sqrt{\frac{\log n}{n}})$, the first phase of Algorithm \ref{alg:alg1} can successfully cluster the nodes in $C$ when $|C|  = \Omega({\frac{\log n}{\epsilon^2}})$
\end{corollary}
}


After the first phase, our algorithm has identified at least $\frac{h(n)}{3}$ vertices belonging to each cluster. In the second phase, we sample $g(n)$ nodes from each of the clusters in $C$.  Let $g(n) \leq \frac{h(n)}{3}$ so that such a sampling is possible. Let the sampled nodes be denoted by $S$ and $S_1=S \sqcap C_1$ and $S_2=S \sqcap C_2$. For each $v \in V\setminus C$, we computes it neighbors in $S_1$ and $S_2$ respectively. If the number of neighbors in $S_1$ is higher than in $S_2$, $v$ is inserted in $C_1$ and otherwise in $C_2$. 


\begin{lemma}\label{lem:gnlemma}
For a node $u\in V\setminus C$, with $g(n) > \min\{\frac{n}{2},\log n \Big(\frac{\sqrt{12B_t(r_d)}+\sqrt{12B_t(r_s)}}{B_t(r_s)-B_t(r_d)}\Big)^{2}\}$, our algorithm correctly identities  the original clusters with probability at least $1-o(1)$. 
% when 
%$\Delta_S = B_t(r_s)g(n) - \sqrt{6\log n g(n)B_t(r_s)}$ and $\Delta_D =  B_t(r_d)g(n) + \sqrt{6\log n g(n)B_t(r_d)}$\end{lemma}
\end{lemma}



\begin{proof}
Consider a node $u \in V \setminus C$. Let without loss of generality $u \in C_1$. Let $Z_1$ and $Z_2$ denote the number of neighbors of $u$ in $S_1$ and $S_2$ respectively. Then $E[Z_1]=B_t(r_s)g(n)$ and $E[Z_2]=B_t(r_d)g(n)$. Applying the Chernoff bound (and then union bound), for all such $u$ with probability at least $1-\frac{1}{n^2}$
\begin{align*}
Z_1 &\geq   B_t(r_s)g(n) - \sqrt{6\log n)g(n)B_t(r_s)}\,\,\text{ and }\\
Z_2  &\leq B_t(r_d)g(n) + \sqrt{6\log n)g(n)B_t(r_d)}
\end{align*}
Therefore, as long as
$$B_t(r_s)g(n) - \sqrt{6\log n)g(n)B_t(r_s)} > B_t(r_d)g(n) + \sqrt{6\log ng(n)B_t(r_d)},$$ vertex $u$ will be classified correctly. This implies, we must have 
\begin{align*}
g(n ) \geq \log n \Big(\frac{\sqrt{6 B_t(r_d)}+\sqrt{6 B_t(r_s)}}{B_t(r_s)-B_t(r_d)}\Big)^{2}
\end{align*}
suffices to cluster all the vertices correctly with probability at least $1-\frac{1}{n}$. If $\log n \Big(\frac{\sqrt{6 B_t(r_d)}+\sqrt{6 B_t(r_s)}}{B_t(r_s)-B_t(r_d)}\Big)^{2} \geq \frac{n}{2}$, then in fact, the second stage is not required as we sample the entire graph in the first phase.
\end{proof}

Note that we set $h(n)=\min\{n,\sqrt{ng(n)}\}$. We now show if $r_s=\Omega\Big((\frac{\log{n}}{n})^{\frac{1}{t}}\Big)$ and $r_s-r_d =\Omega(\min\{r_s, \Big(\frac{\log{n}}{n}\Big)^{\frac{1}{2t}}\})$, then there either exists $\ell_1$ which satisfy the connectivity requirement of RAG (note that either of the two conditions specified for RAG ensure connectivity) as well as the condition of Lemma~\ref{lem:essame-2}. Therefore, our algorithm recovers the clusters correctly in that situation.

%Hence the required query complexity of the entire algorithm is going to be $n g(n) + f^2(n)$.
\begin{theorem*}
[Restatement of Theorem \ref{theorem:main-dense-1}]
If $r_s=\Omega\Big((\frac{\log{n}}{n})^{\frac{1}{t}}\Big)$ and $r_s^t-r_d^t =\Omega( \Big(r_s^t\frac{\log{n}}{h(n)}\Big)^{\frac{1}{2}})$ where $h(n) \geq \frac{\sqrt{6n\log{n}}}{\sqrt{B_t(r_s)}+\sqrt{B_t(r_d)}}$ then our algorithm recovers the clusters correctly by looking at only $O(\min\{n^2, h(n)^2\})$ edges.
\end{theorem*}
\begin{proof}
According to Lemma \ref{lem:essame-2}, our algorithm maintains all edges $(u,v)$ whenever $d(u,v)=\ell$ satisfies the following Cond 1.\begin{align*}
&\frac{h(n)}{2}\Big(\mathcal{V}_t(r_s,r_s,\ell)+\mathcal{V}_t(r_d,r_d,\ell)\Big)- \sqrt{25h(n)\log{n}}\Big(\sqrt{B_t(r_s)} + \sqrt{B_t(r_d)} \Big) > E_S \\
&\text{ or, } \frac{h(n)}{2}\Big(\mathcal{V}_t(r_s,r_s,\ell)+\mathcal{V}_t(r_d,r_d,\ell)\Big)- \sqrt{25h(n)\log{n}}\Big(\sqrt{B_t(r_s)} + \sqrt{B_t(r_d)} \Big) \\
& > h(n)B_t(r_d) + \sqrt{6B_t(r_d)h(n)\log n} \,\text{ take $\theta_s^t=1$}
\end{align*}
Note that the expression on the left is a decreasing function. We consider the maximum value of above expression i.e. when $\ell=0$, assuming $\theta_S^t=1$ and want to show
\begin{align*}
&\frac{h(n)}{2}\Big(B_t(r_s)-B_t(r_d)\Big)>  \sqrt{h(n)\log{n}}\Big(\sqrt{25B_t(r_s)} + \sqrt{25B_t(r_d)} + \sqrt{12B_t(r_d)}\Big) \\
\equiv & \frac{h(n)}{2}\Big(r_s^t - r_d^t)\Big)>  c \sqrt{h(n)\log{n}}\Big(\sqrt{B_t(r_s)} + \sqrt{B_t(r_d)} \Big)
\end{align*}


When $r_s^t - r_d^t = o\Big(\sqrt{\frac{B_t(r_s) \log n}{h(n)}}\Big) = o\Big(\sqrt{\frac{r_s^t \log n}{h(n)}}\Big) $, the expression is violated even for $l=0$.\\

 On the other hand, when $r_s^t - r_d^t = \Omega\Big(\sqrt{\frac{B_t(r_s) \log n}{h(n)}}\Big)$, the above equation is satisfied. Hence, there exists some maximum value of $l$ for which the above mentioned equation (same as Lemma \ref{lem:essame-2}) is satisfied for a suitable choice of $\theta_s^t$. More specifically, if $\ell^t=\Theta(\frac{\log{n}}{n})$, then since both $r_s^t=\Omega((\frac{\log{n}}{n}))$ and $r_d^t=\Omega((\frac{\log{n}}{n}))$, for fixed $t$, $\mathcal{V}_t(r_s,r_s,\ell)=O(r_s^t)$ and $\mathcal{V}_t(r_d,r_d,\ell)=O(r_d^t)$, then both Cond 1 and the connectivity requirements of RAG are satisfied.
 %More specifically  when $r_s^t - r_d^t = \Theta\Big(\sqrt{\frac{B_t(r_s) \log n}{n}}\Big)$, we can simplify the equation to achieve a degree $t$ polynomial 
%\begin{align*}
%&\frac{n}{2}\Big(\mathcal{V}_t(r_s,r_s,\ell)+\mathcal{V}_t(r_d,r_d,\ell)\Big)- \sqrt{25n\log{n}}\Big(\sqrt{B_t(r_s)} + \sqrt{B_t(r_d)} \Big) > nB_t(r_d) + \sqrt{6B_t(r_d)n\log n}  \\
%&\Big(\mathcal{V}_t(r_s,r_s,\ell)+\mathcal{V}_t(r_d,r_d,\ell)\Big) > c \sqrt{\frac{B_t(r_s)\log n}{n}}
%\end{align*}
%Hence, it will have a solution $0\le \ell < \theta \Big(\frac{B_t(r_s)\log n}{n}\Big)^{1/t}$.  Whenever this feasible region of $\ell$ satisfies the RAG connectivity, our algorithm succeeds.
\end{proof}

%\begin{theorem}
%Let $\ell_1$ be defined as 
%\begin{align*}
%& \ell_1=\argmax_{x} \Big(\mathcal{V}_t(r_s,r_s,x)+\mathcal{V}_t(r_d,r_d,x)-2B_t(r_d)\Big)\frac{h(n)}{2} \\
%& >\Big(\sqrt{\mathcal{V}_t(r_s,r_s,x)} + \sqrt{\mathcal{V}_t(r_d,r_d,x)} +\sqrt{3B_t(r_d)}\Big)\sqrt{2h(n)\log n} 
%\end{align*}
%and let $\ell_2$ be defined as
%\begin{align*}
%&\ell_2=\argmin_{x} \frac{h(n)}{2}\Big(2\mathcal{V}_t(r_s,r_d,r_d)-\mathcal{V}_t(r_s,r_s,x)-\mathcal{V}_t(r_d,r_d,x)\Big) \\
%&>\sqrt{2h(n)\log n}\Big(\sqrt{\mathcal{V}_t(r_s,r_s,x)} +\sqrt{\mathcal{V}_t(r_d,r_d,x)}+\sqrt{3B_t(r_d)}\Big)
%\end{align*}
%If $\ell_1^t = \omega\Big(\frac{\log n}{c_t n}\Big)$ or $r_s^t -\ell_2^t =\omega \Big(\frac{\log n}{c_t n}\Big)$, then the query complexity is going to be 
%\begin{align*}
%n \log n \Big(\frac{\sqrt{6B_t(r_d)}+\sqrt{6B_t(r_s)}}{B_t(r_s)-B_t(r_d)}\Big)^{2}
%\end{align*}
%\end{theorem}
%
%\begin{proof}
%The proof follows from the fact that if the subgraph restricted to the $h(n)$ nodes and the edges such that the distance of the edges satisfy the conditions of Theorem \ref{th:main1d} is connected, then our algorithm \ref{alg:alg1} is successfully able to classify the $h(n)$ nodes exactly. Using the results from connectivity of the Random Annulus Graph from Theorem \ref{thm:highdem}, we get the statement of the theorem. Recall that we set $h(n)=\sqrt{ng(n)}$ and therefore the query complexity simply follows by substituting the expression for $g(n)$ from Lemma \ref{lem:gnlemma}.
%\end{proof}


\begin{corollary}
 When $r_s$ and $r_d$ are constant with $r_s^t-r_d^t = \epsilon^t$ and $\epsilon^t=\Omega\Big(\sqrt{\frac{\log n}{n}}\Big)$ then our algorithm maintains only $O(\frac{n\log n}{\epsilon^{2t}})$ edges.
\end{corollary}
\begin{proof}
Consider $t=1$. From Theorem~\ref{theorem:main-dense-1}, $\epsilon$ must satisfy $\epsilon=\Omega(\Big(\frac{\log{n}}{h(n)}\Big)^{\frac{1}{2}}$. By setting $h(n)=\frac{\sqrt{n\log n}}{\epsilon}$, we get $\epsilon=\Omega\Big(\sqrt{\frac{\log n}{n}}\Big)$. Thus our algorithm maintains only $\frac{n\log{n}}{\epsilon^2}$ edges. Similarly, for any dimension $t$, if $r_s^t-r_d^t=\epsilon^t=\Omega\Big(\sqrt{\frac{\log n}{n}}\Big)$ then our algorithm only maintains $\frac{n\log{n}}{\epsilon^{2t}}$ edges.
\end{proof}





==> rgg-gbm.tex <==
\section{The Geometric Block Model: Details}
\label{sec:gbm-detail}

\subsection{Immediate consequence of VRG connectivity}
The following lower bound for GBM can be obtained as a  consequence of Theorem~\ref{thm:rag}.

\begin{theorem*}(\ref{gbm:lower})[Impossibility in GBM]
Any algorithm to recover the partition in ${\rm GBM}(\frac{a \log n}{n},\frac{b \log n}{n})$ will give incorrect output with probability $1-o(1)$ if $a-b < 0.5$ or $a < 1$.
\end{theorem*}
\begin{proof}
%\textcolor{red}{This part should be corrected, may be by adding the multi component proof in the appendix} 
%Recall that an edge between $2$ nodes $u$ and $v$ in the $2$-cluster GBM was formed if the associated random variables $X_u$ and $X_v$ uniformly chosen from $[0,1]$ are close in Lee distance. 
Consider the scenario that not only the geometric block model graph  ${\rm GBM}(\frac{a \log n}{n},\frac{b \log n}{n})$ was provided to us, but also the random values $X_u \in [0,1]$ for all vertex $u$ in the graph were provided. We will show that we will still not be able to recover the correct partition of the vertex set $V$ with probability at least $0.5$ (with respect to choices of $X_u,~u, v\in V$ and any randomness in the algorithm).

In this situation, the edge $(u,v)$ where $d_L(X_u,X_v) \le \frac{b \log n}{n}$ does not give any new information than $X_u,X_v$. However the edges $(u,v)$ where $\frac{b \log n}{n} \le d_L(X_u,X_v) \le \frac{a \log n}{n}$ are informative, as existence of such an edge will imply that $u$ and $v$ are in the same part. These edges constitute a vertex-random graph ${\rm VRG}(n, [\frac{b \log n}{n},\frac{a \log n}{n}])$. But if there are more than two components in this vertex-random graph, then it is impossible to separate out the vertices into the correct two parts, as the connected components can be assigned to any of the two parts and the VRG along with the location values ($X_u, u \in V$) will still be consistent. 

What remains to be seen that ${\rm VRG}(n, [\frac{b \log n}{n},\frac{a \log n}{n}])$ will have $\omega(1)$ components with high probability  if $a-b < 0.5$ or $a < 1$. This is certainly true when $a-b < 0.5$ as we have seen in Theorem~\ref{thm:lower_bound}, there can indeed be $\omega(1)$ isolated nodes with high probability. On the other hand, when $a<1$, just by using an analogous argument it is possible to show that there are $\omega(1)$ vertices that do not have any neighbors on the left direction (counterclockwise). We delegate the proof of this claim as Lemma \ref{lem:disc} in the appendix.  %\textcolor{red}{Give  this proof in  appendix?} 
If there are $k$ such vertices, there must be at least $k-1$ disjoint candidates.This completes the proof.
\end{proof}

%\textcolor{red}{Fill up the corollary below} 



\begin{theorem}[GBM with known vertex locations]\label{thm:gbmplus}
Suppose a geometric block model graph ${\rm GBM}(\frac{a \log n}{n},\frac{b \log n}{n})$ is provided along with the associated  values of the locations $X_u$ for every vertex $u$. Any algorithm to recover the partition in ${\rm GBM}(\frac{a \log n}{n},\frac{b \log n}{n})$ will give incorrect output with probability $1-o(1)$ if $a-b < 0.5$ or $a < 1$. On the other hand it is possible to recover the partition exactly with probability $1-o(1)$ when $a-b > 0.5$ and $a > 1$.
\end{theorem}
\begin{proof}
We need to only prove that  it is possible to recover the partition exactly with probability $1-o(1)$ when $a-b > 0.5$ and $a > 1$, since the other part is immediate from Theorem~\ref{gbm:lower}. For any pair of vertices $u,v$, we can verify if $d(u,v) \in [\frac{b \log n}{n},\frac{a \log n}{n}]$. If that is the case then by just checking in the GBM graph whether they are connected by an edge or not we can decide whether they belong to the same cluster or not respectively. What remains to be shown that  all vertices can be covered by this procedure. However that will certainly be the case since ${\rm VRG}(n , [\frac{b \log n}{n},\frac{a \log n}{n}])$ is connected with high probability.
\end{proof}

%Next we provide the main algorithm for recovery in GBM and its analysis.


